Optimizing Through Learned Errors for Accurate Sports Field Registration

We propose an optimization-based framework to register sports field templates onto broadcast videos. For accurate registration we go beyond the prevalent feed-forward paradigm. Instead, we propose to train a deep network that regresses the registration error, and then register images by finding the registration parameters that minimize the regressed error. We demonstrate the effectiveness of our method by applying it to real-world sports broadcast videos, outperforming the state of the art. We further apply our method on a synthetic toy example and demonstrate that our method brings significant gains even when the problem is simplified and unlimited training data is available.

==> tbl/hockey/item.tex <==
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{table*}
\begin{center}
\scriptsize
\begin{tabularx}{\linewidth}{l C C C C}
    \toprule
      & \multicolumn{2}{c}{mIoU$_{\text{whole}}$} & \multicolumn{2}{c}{mIoU$_{\text{part}}$} \\
      & mean & median & mean & median \\
     \midrule
     ~\cite{Homayounfar17d} \textsuperscript{\ref{ft:uot}} & 82.0 & -- & -- & -- \\
     \midrule
     Initial reg. only & 86.5 & 87.3 & 90.4 & 91.0 \\
     Feed-forward ref. & 93.0 & 94.0 & 96.0 & 96.8 \\
     NN & N/A & N/A & N/A & N/A \\
     NN + optim. & N/A & N/A & N/A & N/A \\
     Joint training & -- & -- & -- & -- \\
     IOUpart & 95.6 & 96.6 & 97.3 & 98.3 \\
     IOUwhole & {\bf96.2} & {\bf97.0} & {\bf97.6} & {\bf98.4} \\
     Reproj & 94.9 & 95.5 & 97.1 & 97.6 \\
     \bottomrule
\end{tabularx}
\begin{tabularx}{\linewidth}{l C C C C C C C C C C C}
    \toprule
      & ~\cite{Homayounfar17d} \textsuperscript{\ref{ft:uot}} & ~\cite{Sharma18d} & ~\cite{Chen18e} & Initial reg. only &  Feed-forward ref. & NN & NN + optim. & Joint training & IOUpart & IOUwhole & Reproj\\
     mean & 82.0 & -- & -- & 86.5 & 93.0 & N/A & N/A & -- & 95.6 & 96.2 & 94.9 \\
     median & -- & -- & -- & 87.3 & 94.0 & N/A & N/A & -- & 96.6 & 97.0 & 95.5\\
     mean &  -- & -- & -- & 90.4 & 96.0 & N/A & N/A & -- & 97.3 & 97.6 & 97.1 \\
     median & -- & -- & -- & 91.0 & 96.8 & N/A & N/A & -- & 98.3 & 98.4 & 97.6 \\
     \bottomrule
\end{tabularx}
\end{center}
\caption{
  \TODO{Transpose the table, merge with worldcup}
Results for the Hockey dataset. 
Best results are in bold. 
Results for ~\cite{Homayounfar17d} is taken from the original paper.
Our method performs best.
}
\label{tbl:hockey}
\end{table*}



==> tex/method_network.tex <==
\subsection{Networks}


\paragraph{Initial registration network.}
Following a recent trend~\cite{Ren15, He17},
we base our network on the ResNet-18 architecture~\cite{He16}.
Instead of the classification head, we simply replace the last fully connected layer to estimate 8 numbers \wj{which represent the homography, $\bh$}.%, that is, our homography parameterization.
We use the pretrained weights for the network trained on ImageNet~\cite{Deng09}, and fine-tune.


\paragraph{Registration error network.}
For the registration error network, we also rely on the ResNet-18 architecture, but with spectral normalization~\cite{Miyato18} on all convolutional layers, and take as input a 6-channel image, that is, the concatenation of the input image and the warped target \template{}. Spectral normalization smooths the error predictions by constraining the Lipschitz constant of the model, which limits the magnitude of its gradients.
\wj{As the output of the registration error network cannot be negative, we use sigmoid function as the final activation function for the IoU based error metrics, and squaring function for reprojection error metric.}
For the registration network, as the input is very different from a typical image-based network, we train from scratch.







==> tex/results_ablation.tex <==

\subsection{Ablation study}
\label{sec:ablation}

\ky{
average reprojection error for all visible points, when projected to the template with the groundtruth homography and projected back to the image with the perturbed homogrpahy.
}



\paragraph{Number of optimization iterations.}

In \fig{itervsiou} we show a qualitative example on how the number of optimization steps affect the final registration.
The overall summary on the entire dataset is provided in \fig{itervsiou_summary}.
As more optimization iterations are spent, the registration accuracy becomes higher.

As shown in \fig{itervsiou_summary}, the enhancement through optimization is more prominent in the WorldCup dataset as the initial registration network performs poorly on this dataset, due to the lack of training data.
On the other hand, even with small amount of training data, we are able to use the proposed registration error network to obtain enhanced registration results.

\paragraph{Spectral normalization.}

\label{sec:specnorm}

To demonstrate the importance of spectral normalization, we conduct a study where we investigate the optimization paths on the error surface provided by registration error network.
For ease in visualization, we consider only the translation.
In more detail, we warp the sports field model according to the ground-truth homography, then translate them in a grid setup and retrieve the estimated errors at these locations.
We then select a random position and start optimizing with various optimization methods.
We use vanila SGD to demonstrate demonstrate the immediate effect of gradients, ADAM for showing how the actual pipeline would performs, L-BFGS~\todo{\cite{liu89} } as a representative quasi-newton optimizer, and PSO~\todo{\cite{Kennedy10}} to show how gradient-free methods perform.

As shown in \fig{optandspec}, all gradient-based methods, SGD, ADAM, and L-BFGS fail when the error networks is trained without spectral normalization.
Note that the smoothness of the error surface do not differ greatly in both cases yet a drastic difference is caused.
Step size is also not the main reason, as L-BFGS also fails.
We suspect that this could be because spectral normalization enforces the network to be less dependant on particular feature map responses, thus making the network insensitive to small local changes within the image.
Further theoretical study on this phenomena would be beneficial as future work.

Given that PSO is impractical for time-critical application, spectral norm is an essential component that allows using the registration error network for optimization. 


